JavaVulBench: A Java Vulnerability Benchmark with Realistic Splits, a Unified Multi-Backend Harness, and a Leakage-Aware Evaluation Mode

We release \textsc{JavaVulBench}, a benchmark dataset and evaluation harness for Java vulnerability detection. The dataset contains $\sim$30{,}600 Java methods spanning 1{,}740 CVEs and 700+ projects, labelled at both method and line granularity, with per-CVE publication dates and five realistic split strategies: random, project-disjoint, temporal, deduplicated, and unseen CWE-family. The harness provides a single \texttt{LlmPrediction} schema across three backend families (encoder classifiers, local generative models served by Ollama, and API-served LLMs routed through OpenRouter) so that twelve reference detectors CodeBERT, GraphCodeBERT, UniXcoder, DeepSeek-Coder-1.3B, and eight API/open-weight LLMs (GPT-4o, GPT-4.1-mini, Claude Sonnet~4, DeepSeek-v3, DeepSeek-Coder-v2, Qwen-2.5-Coder-14B/7B, CodeLlama-13B) are evaluated under identical conditions from a single command. A pre-training contamination audit is shipped alongside every model so users can separate genuinely unseen test CVEs from potentially memorised ones. Data, code, and fine-tuned checkpoints are archived on Zenodo [31] and short demonstration video is available on YouTube (https://www.youtube.com/watch?v=nMTX\_hqkuoM) https://www.youtube.com/watch?v=nMTX_hqkuoM.

==> figs/fig_prompt_strategy.tex <==
% Mean F1 per API LLM averaged across the five shipped splits, broken out
% by prompt strategy. Numbers from results/main_results.csv.
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
  ybar=2pt,
  bar width=5pt,
  width=\columnwidth,
  height=4.4cm,
  enlarge x limits=0.18,
  ymin=0, ymax=0.55,
  ylabel={Mean F1 (across splits)},
  symbolic x coords={GPT-4o,Claude Sonnet 4,DeepSeek-v3,GPT-4.1-mini,Qwen-14B},
  xtick=data,
  x tick label style={rotate=20,anchor=east,font=\footnotesize},
  tick label style={font=\footnotesize},
  ylabel style={font=\footnotesize},
  legend style={font=\footnotesize,at={(0.02,0.98)},anchor=north west,
                draw=none,fill=none,column sep=4pt,legend columns=3},
]
\addplot+[fill=cyan!60!white,draw=cyan!60!black] coordinates {
  (GPT-4o,0.380) (Claude Sonnet 4,0.369) (DeepSeek-v3,0.306) (GPT-4.1-mini,0.294) (Qwen-14B,0.276)
};
\addplot+[fill=magenta!50!white,draw=magenta!60!black] coordinates {
  (GPT-4o,0.351) (Claude Sonnet 4,0.378) (DeepSeek-v3,0.202) (GPT-4.1-mini,0.165) (Qwen-14B,0.224)
};
\addplot+[fill=yellow!75!black,draw=olive!70!black] coordinates {
  (GPT-4o,0.348) (Claude Sonnet 4,0.401) (DeepSeek-v3,0.305) (GPT-4.1-mini,0.245) (Qwen-14B,0.309)
};
\legend{zero-shot,few-shot,RAG}
\end{axis}
\end{tikzpicture}
\caption{Prompt-strategy comparison for the five API-served LLMs on
which all three strategies (zero-shot, few-shot, RAG) were run. Values
are mean detection F1 across the five splits shipped with JavaVulBench.
RAG helps the stronger generalists (Claude, DeepSeek-v3, Qwen-14B) but
not GPT-4o; few-shot hurts weaker models. The harness lets users
replicate this comparison on their own prompt template.}
\label{fig:prompts}
\end{figure}


==> figs/fig_split_impact.tex <==
% F1 across the four shipped splits for every fine-tuned reference model.
% Numbers are taken from results/metrics/*.json (fine_tuned > lora > zero_shot).
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
  ybar=2pt,
  bar width=4pt,
  width=\columnwidth,
  height=4.4cm,
  enlarge x limits=0.18,
  ymin=0, ymax=0.55,
  ylabel={Detection F1},
  symbolic x coords={CodeBERT,GraphCodeBERT,UniXcoder,DeepSeek-Coder-1.3B},
  xtick=data,
  x tick label style={rotate=20,anchor=east,font=\footnotesize},
  tick label style={font=\footnotesize},
  ylabel style={font=\footnotesize},
  legend style={font=\footnotesize,at={(0.02,0.98)},anchor=north west,
                draw=none,fill=none,column sep=4pt,legend columns=2},
  nodes near coords style={font=\tiny,rotate=90,anchor=west},
]
\addplot+[fill=blue!60!white,draw=blue!60!black] coordinates {
  (CodeBERT,0.422) (GraphCodeBERT,0.343) (UniXcoder,0.446) (DeepSeek-Coder-1.3B,0.341)
};
\addplot+[fill=orange!80!white,draw=orange!70!black] coordinates {
  (CodeBERT,0.000) (GraphCodeBERT,0.256) (UniXcoder,0.298) (DeepSeek-Coder-1.3B,0.062)
};
\addplot+[fill=green!60!white,draw=green!55!black] coordinates {
  (CodeBERT,0.000) (GraphCodeBERT,0.097) (UniXcoder,0.171) (DeepSeek-Coder-1.3B,0.335)
};
\addplot+[fill=red!60!white,draw=red!55!black] coordinates {
  (CodeBERT,0.118) (GraphCodeBERT,0.159) (UniXcoder,0.345) (DeepSeek-Coder-1.3B,0.000)
};
\legend{Random,Project,Time,CWE-family}
\end{axis}
\end{tikzpicture}
\caption{Detection F1 of every shipped fine-tuned reference model on
each of the four split strategies (full test sets). The gap between
\emph{random} and \emph{project-disjoint} quantifies the leakage
headroom researchers should expect if they choose an optimistic split;
DeepSeek-Coder-1.3B was not fine-tuned on the CWE-family split and is
reported as --.}
\label{fig:split}
\end{figure}


==> tables/perfomance.tex <==
\begin{table}[t]
  \centering
  \caption{End-to-end runtimes for the \textsc{JavaVulBench} pipeline
  on Windows~11, Python~3.12, CUDA~12.8, an RTX 3060/4060-class GPU
  (8--12\,GB VRAM), and 16\,GB RAM. ``Cached'' uses the shipped mining
  artifacts; ``From scratch'' rebuilds all artifacts.}
  \label{tab:pipeline-runtime}

  \scriptsize
  \setlength{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{0.95}

  \begin{tabularx}{\linewidth}{@{}cXcc@{}}
    \toprule
    \textbf{Stage} & \textbf{Step} & \textbf{Cached} & \textbf{From scratch} \\
    \midrule
    0 & Inspect artifacts on disk
      & instant
      & instant \\

    1 & Mining: CVE $\rightarrow$ commit $\rightarrow$ source
      & --
      & 6--10\,h \\

    2 & Build benchmark (\texttt{--stats})
      & $\sim$5\,s
      & 10--20\,min \\

    3 & Inspect one sample
      & instant
      & instant \\

    4 & Enumerate the five splits
      & instant
      & instant \\

    5 & Pre-training contamination audit
      & 30--90\,s
      & 30--90\,s \\

    6 & Fine-tune \texttt{unixcoder-base}
      & 3--5\,min
      & 3--5\,min \\

      & \quad fallback: GPT-4.1-mini, 20 samples
      & 20--40\,s
      & 20--40\,s \\

      & \quad same fine-tune on CPU only
      & 45--75\,min
      & 45--75\,min \\

    7 & Build paper tables
      & $<$10\,s
      & $<$10\,s \\
    \midrule
    \multicolumn{2}{@{}l}{\textbf{Total pipeline}}
      & \textbf{30--45\,min}
      & \textbf{8--12\,h} \\
    \bottomrule
  \end{tabularx}
\end{table}

==> tables/table_leakage_metrics.tex <==
% VS4: leakage-aware F1 on the clean (post-pretrain-cutoff) subset
\begin{table}[t]
\centering\small
\caption{Leakage-aware detection on the \emph{time} split (API-LLM probe,
$N=200$). \emph{Risky} = test CVEs published before the model's
pre-training cutoff (potentially memorised); \emph{Clean} = CVEs
published after (guaranteed unseen). The audit partitions the test set
per model, and F1 on the clean subset is the memorisation-free number.}
\label{tab:leakage_metrics}
\begin{tabular}{lcccc}
\toprule
Model & F1$_{\text{all}}$ & F1$_{\text{clean}}$ & $N_{\text{clean}}$ & $N_{\text{risky}}$ \\
\midrule
GPT-4o              & 0.488 & 0.528 & 174 &  26 \\
GPT-4.1-mini        & 0.296 & 0.323 & 115 &  85 \\
Claude Sonnet 4     & 0.444 & 0.480 &  74 & 126 \\
DeepSeek-v3         & 0.302 & 0.286 & 109 &  91 \\
DeepSeek-Coder-v2   & 0.152 & 0.213 & 117 &  83 \\
Qwen-2.5-Coder-14B  & 0.207 & 0.270 & 132 &  68 \\
Qwen-2.5-Coder-7B   & 0.138 & 0.186 & 132 &  68 \\
CodeLlama-13B       & 0.331 & 0.331 & 200 &   0 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_rq3.tex <==
% VS3: per-CWE macro-recall (families the model ever gets right on the probe)
\begin{table}[t]
\centering\small
\caption{Per-CWE behaviour of the API LLMs on the project-disjoint probe,
across the 15 CWE families represented in the subset. Macro-recall averages
recall over families; \emph{families hit} counts families with at least one
correctly flagged vulnerable method. The spread from Claude Sonnet 4 to
GPT-4.1-mini shows that \emph{which} CWEs an LLM recognises is itself a
measurable dimension the benchmark exposes.}
\label{tab:rq3}
\begin{tabular}{lcc}
\toprule
Model & Macro-recall & Families hit \\
\midrule
Claude Sonnet 4     & 0.539 & 12 / 15 \\
GPT-4o              & 0.311 &  9 / 15 \\
DeepSeek-v3         & 0.161 &  5 / 15 \\
Qwen-2.5-Coder-14B  & 0.161 &  6 / 15 \\
GPT-4.1-mini        & 0.056 &  2 / 15 \\
\bottomrule
\end{tabular}
\end{table}

